Variance-reduced Zeroth-Order Methods for Fine-Tuning Language Models

Fine-tuning language models (LMs) has demonstrated success in a wide array of downstream tasks. However, as LMs are scaled up, the memory requirements for backpropagation become prohibitively high. Zeroth-order (ZO) optimization methods can leverage memory-efficient forward passes to estimate gradients. More recently, MeZO, an adaptation of ZO-SGD, has been shown to consistently outperform zero-shot and in-context learning when combined with suitable task prompts. In this work, we couple ZO methods with variance reduction techniques to enhance stability and convergence for inference-based LM fine-tuning. We introduce Memory-Efficient Zeroth-Order Stochastic Variance-Reduced Gradient (MeZO-SVRG) and demonstrate its efficacy across multiple LM fine-tuning tasks, eliminating the reliance on task-specific prompts. Evaluated across a range of both masked and autoregressive LMs on benchmark GLUE tasks, MeZO-SVRG outperforms MeZO with up to 20% increase in test accuracies in both full- and partial-parameter fine-tuning settings. MeZO-SVRG benefits from reduced computation time as it often surpasses MeZO's peak test accuracy with a $2\times$ reduction in GPU-hours. MeZO-SVRG significantly reduces the required memory footprint compared to first-order SGD, i.e. by $2\times$ for autoregressive models. Our experiments highlight that MeZO-SVRG's memory savings progressively improve compared to SGD with larger batch sizes.

==> misc.tex <==
% \subsection{Solving Least-Squares (100-dimensional)}
% We find that MeZO-SVRG exhibits improved convergence properties over MeZO. We demonstrate this by solving the LS problem 
%     \begin{align}\label{eq:ls}
%         \min_{w\in\R^d} \|Xw-y\|_2^2,
%     \end{align}
% where $X\in\R^{n\times d}$ is a randomly sampled dataset, $w\in\R^d$ is fixed a priori and $y\in\R^n := Xw +\textrm{noise}$ is the target vector. In our experiment we focus on the 100-dimensional problem, i.e. with $d=100$ and $n=1000$. Details of the experiments hyperparameters are summarized in Appendix . Figure illustrates the improved MeZO-SVRG convergence performance.

% \subsection{MNIST Classification with Multi-layer Perceptron (25K-dimensional)}
% Next, we scale up in complexity and consider the MNIST classification problem with a two-hidden layer MLP. Specifically, we train a MLP with 32 and 16 hidden units in its respective layers. This model has approximately $25000$ parameters.

% As before, we perform a coarse search over the hyperparameter grid summarized in Table \ref{tab:hyperparameters}. 

% Figures \ref{fig:MNISTquery} and \ref{fig:MNISTquery} again demonstrate ZO-SVRG's improved convergence performance of MeZO. As with LS, we observe that ZO-SVRG is able to converge to a training loss that MeZO is unable to reach.


%In the preliminary experiments reported in \citet{malladi2023mezo}, authors show that the inclusion of a simple prompt is crucial for MeZO to succeed. Prior works have demonstrated how the inclusion of a suitable prompt ensures that the fine-tuning objective is closely related to the pre-training one \citep{saunshi2021a, malladi2023kernelbased}. However, as has been shown in other work, crafting suitable prompts is a difficult task. Thus, we would like ZO methods to work without the need to include such prompts. In this section, we implement the considered methods under both scenarios: with and without adding any prompts. We demonstrate ZO-SVRG's superior performance under both regimes.

\begin{table*}[h!]
\centering
\begin{tabular}{l|c c|c c c}
\toprule
 & \multicolumn{2}{c|}{\textbf{LS}} & \multicolumn{3}{c}{\textbf{MNIST}} \\
%\cline{2-6}
\textbf{Method} & Training Loss  & Queries & Training Loss  & Test Accuracy (\%) & Queries \\
\hline
MeZO & - & - & - & - & - \\
ZO-SVRG & - & - & - & - & - \\
FO-SGD & - & - & - & - & - \\
\bottomrule
\end{tabular}
\caption{Results for the LS and MNIST classification problems.}
\label{tab:LSMNIST}
\end{table*}



\newpage
\section{Additional Results for LS Experiments}


\begin{figure*}[ht]
    \centering
    \begin{minipage}{0.45\columnwidth}
        \includegraphics[width=0.8\linewidth]{figs/LS (n=1000, d=100).pdf}
        \subcaption{}
        \label{fig:LSiteration}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\columnwidth}
        \includegraphics[width=0.8\linewidth]{figs/LS (n=1000, d=100): Query Complexity.pdf}
        \subcaption{}
        \label{fig:LSquery}
    \end{minipage}
    \caption{Illustrates ZO-SVRG's improved convergence performance over MeZO when solving the LS problem. In (a) we show the iteration complexity while (b) shows the query complexity.}
\end{figure*}

\newpage
\section{Additional Results for MNIST Classification Experiments}

\begin{figure*}[ht]
    \centering
    \begin{minipage}{0.45\columnwidth}
        \includegraphics[width=0.9\linewidth]{figs/MNIST: Iteration Complexity.pdf}
        \subcaption{}
        \label{fig:MNISTiteration}
    \end{minipage}
    \hfill
    \begin{minipage}{0.45\columnwidth}
        \includegraphics[width=0.9\linewidth]{figs/MNIST: Query Complexity.pdf}
        \subcaption{}
        \label{fig:MNISTquery}
    \end{minipage}
    \caption{Illustrates ZO-SVRG's improved convergence performance over MeZO when training an two-layer MLP for MNIST classification. In (a) we show the iteration complexity while (b) shows the query complexity.}
\end{figure*}


\begin{table*}[ht]
	\centering
	\caption{Experiments on DistilBERT (with 512 samples). Here Adapter refers to fine-tuning the last transformer block and classification head of the model. FO refers to first-order methods and ZO refers to zeroth-order. Unless otherwise specified this table summarizes results for full parameter fine-tuning.}\vspace{1em}
 {
 \scriptsize
	\begin{tabularx}{0.85\linewidth}{l | l | c c c c }
	\toprule
 \textbf{Task} & \textbf{Method} & Training Loss ($10^{-1}$)$\downarrow$ & Validation Accuracy (\%)$\uparrow$ & Queries ($\times 10^6$)$\downarrow$ & Max Memory Usage (GB)$\downarrow$\\
	\toprule %
	%
 & MeZO  & 10.76 & 34.4 & 1.02\\
 & MeZO (Adapter)  & 10.77 & 32.8 & 1.02\\
 MNLI & ZO-SVRG  & \textbf{8.049} & \textbf{55.46} & 10.8\\
 & ZO-SVRG (Adapter)  & \textbf{10.41} & \textbf{42.18} & 10.8\\
  \hdashline
   & FO-SGD  & 0.0042  & 61.7 & 1.02\\
 & FO-SGD (Adapter)  & 13.63 & 50 & 1.02\\
 % \toprule\\
 %  & MeZO  &  & - & --\\
 % & MeZO (Adapter)  &  & - & --\\
 % QNLI & ZO-SVRG  &  & - & --\\
 % & ZO-SVRG (Adapter)  &  & - & --\\
 %   & FO-SGD  & 0.013 & 75.19 & 1822\\
 % & FO-SGD (Adapter)  & 6.321 & 54 & 1825\\
 % \toprule\\
 %  & MeZO  &  & - & --\\
 % & MeZO (Adapter)  &  & - & --\\
 % SST-2 & ZO-SVRG  &  & - & --\\
 % & ZO-SVRG (Adapter)  &  & - & --\\
 %   & FO-SGD  & 0.016 & 86.32 & 1614\\
 % & FO-SGD (Adapter)  & 2.972 & 80.27 & 1614\\
 % \toprule\\
 %   & MeZO  &  & - & --\\
 % & MeZO (Adapter)  &  & - & --\\
 % CoLA & ZO-SVRG  &  & - & --\\
 % & ZO-SVRG (Adapter)  &  & - & --\\
 %   & FO-SGD  & 0.376 & 72 & 1814\\
 % & FO-SGD (Adapter)  & 5.767 & 71 & 1816\\
 \bottomrule
	\end{tabularx}
	}
	\label{tab:distilbertresultsshort}
\end{table*}


\begin{enumerate}
    \item We propose a Memory Efficient ZO stochastic variance-reduced gradient (MeZO-SVRG) method that we demonstrate empirically outperforms the existing MeZO \citep{malladi2023mezo}. MeZO-SVRG mitigates some notable drawbacks of MeZO by combining iterates that utilize fullbatch and minibatch information \prraman{vague, not clear what information you refer to}.
    \item We evaluate the proposed MeZO-SVRG method on a variety of models, including Roberta-large and GPT2, on benchmark GLUE tasks, and find that ZO-SVRG consistently outperforms MeZO and reduces the gap compared to first-order SGD (FO-SGD) whilst maintaining a memory footprint equivalent to inference passes \prraman{how much is this memory footprint, would be good to be specific}.
    \item We develop theory \prraman{same comment as above, it is vague, need to mention what improved rate we obtained} that supports MeZO-SVRG's improved convergence properties over MeZO in the fine-tuning setting.
\end{enumerate}

We demonstrate empirically that MeZO-SVRG outperforms MeZO consistently on a variety of LLM fine-tuning tasks and requires significantly less GPU hours to achieve this performance. Furthermore, we show that across model types and fine-tuning tasks MeZO-SVRG is able to considerably close the performance gap while benefiting from a $2\times$ reduction in memory utilization. 


\subsection{Understanding MeZO-SVRG Hyperparameters}
% \prraman{This sub-section title is not informative, maybe it is ok if we move to appendix, but if you keep in main body then better to say what kind of ablations you are referring to.}
% \youngsuk{Ablation study goes to the last}
We aim to better understand how the role of the perturbation scale $\mu$ in computing SPSA estimators as well as regularity of full-batch update steps impacts the MeZO-SVRG performance. Appendix \ref{appendix:ablations} provides a detailed overview of our ablation studies. We perform ablation studies with the DistilBert model on the MNLI \citep{williams2018broadmnli} dataset.

\textbf{Varying Perturbation Scale.} We find that beyond a sufficiently small setting of $\mu$, we observe no noticeable performance gains for MeZO-SVRG. This is in line with findings in \citet{malladi2023mezo} and theory which suggests that the SPSA estimator is asymptotically unbiased in with respect to $\mu$ \citep{spsa}. Based on this finding we use the same default value of $\mu=1e-3$ as proposed in \citet{malladi2023mezo}. Due to space limitations, the empirical comparisons of different settings of $\mu$ are provided in Appendix \ref{appendix:perturbation}.

\textbf{Varying $\mathbf{q}$.} The setting of $q$ in Algorithm \ref{alg:method2} is critical to the performance of MeZO-SVRG. In Appendix \ref{appendix:q}, we investigate different configurations of hyperparameter $q$. Smaller settings of $q$ mean that more updates are done with full-batch SPSA estimators. A greater frequency of full-batch steps improves the convergence rate. However, we also find that mixing full-batch and mini-batch updates ($q\geq 2$) lends greater stability to the algorithm than solely performing full-batch updates ($q=1$).


\begin{figure*}[h]
    \centering
    \begin{minipage}{0.6\columnwidth}
    \centering
        \includegraphics[width=\linewidth]{figs/Memory_Usage.pdf}
        \subcaption{}
        \label{fig:memoryusage}
    \end{minipage}
    \hfill
    \begin{minipage}{1.35\columnwidth}
    \centering{\scriptsize
            % \begin{tabular}{lcccccc}
            % \toprule
            %  & \multicolumn{2}{c}{\textbf{Largest OPT/GPT that can fit}} & \multicolumn{4}{c}{\textbf{Memory Usage (GB) for RoBERTa-large}}  \\
            % \cmidrule{2-3} \cmidrule{4-7}
            %   \textbf{Method}  & 1$\times$A100 (40GB)    &  1$\times$H100 (80GB) & $\textrm{bs}=8$ & $\textrm{bs}=16$& $\textrm{bs}=32$& $\textrm{bs}=64$ \\
            % \midrule
            % MeZO   & 6.7B  & 15B & 1.99 (58\%) & 2.07 (69\%) & 2.21 (79\%) & 2.51 (88\%) \\
            % MeZO-SVRG   & 2.7B   & 6.7B & 4.22 (9\%) & 4.36 (35\%) & 4.51 (58\%) & 4.72 (76\%)\\
            %  FO-SGD   & 1.6B   & 2.7B  & 4.66 & 6.74 & 10.67 & 18.55\\
            % \bottomrule
            % \end{tabular}}
            % \subcaption{}
            % \label{tab:memory}
            \begin{tabular}{lccccc}
            \toprule
             & \multicolumn{2}{c}{\textbf{Largest OPT/GPT that can fit}} & \multicolumn{3}{c}{\textbf{Memory Usage (GB) for RoBERTa-large}}  \\
            \cmidrule{2-3} \cmidrule{4-6}
              \textbf{Method}  & 1$\times$A100 (40GB)    &  1$\times$H100 (80GB) & $\textrm{bs}=16$& $\textrm{bs}=32$& $\textrm{bs}=64$ \\
            \midrule
            MeZO   & 6.7B  & 15B & 2.07 (69\%) & 2.21 (79\%) & 2.51 (88\%) \\
            MeZO-SVRG   & 2.7B   & 6.7B  & 4.36 (35\%) & 4.51 (58\%) & 4.72 (76\%)\\
             FO-SGD   & 1.6B   & 2.7B  & 6.74 & 10.67 & 18.55\\
            \bottomrule
            \end{tabular}}
            \subcaption{}
            \label{tab:memory}
            % \begin{tabular}{lccccccc}
            % \toprule
            %  & \multicolumn{3}{c}{\textbf{Memory Usage (GB) for Autogressive Models}} & \multicolumn{4}{c}{\textbf{Memory Usage (GB) for RoBERTa-large}}  \\
            % \cmidrule{2-4} \cmidrule{5-8}
            %   \textbf{Method}  & GPT2 (1.6B)    &  OPT-2.7B & OPT-6.7B & $\textrm{bs}=16$& $\textrm{bs}=32$& $\textrm{bs}=64$ \\
            % \midrule
            % MeZO   & x  & x & x & 1.99 (58\%) & 2.07 (69\%) & 2.21 (79\%) & 2.51 \\
            % MeZO-SVRG   & x  & x & x & 4.22 (9\%) & 4.36 (35\%) & 4.51 (58\%) & 4.72\\
            %  FO-SGD   & x & x & x  & 4.66 & 6.74 & 10.67 &\\
            % \bottomrule
            % \end{tabular}}
            % \subcaption{}
            % \label{tab:memory}
    \end{minipage}
    \caption{(a) We measure the minimum memory usage for the different methods on the autoregressive models ($\textrm{batch size (bs)}=1$ and input length is set to max context length of model). MeZO-SVRG yields a $2\times$ improvement over FO-SGD in terms of memory utilization.  (b) We show the largest autoregressive models that can fit on GPUs with 40 and 80GB memory. We also measure the memory usage under different batch sizes (bs) when fine-tuning RoBERTa-large \citep{robertalarge} with the methods. The percentages in the parentheses indicate the memory savings with respect to FO-SGD.}
\end{figure*}

